View-Dependent Displays and the Space of Light Fields

In this paper we explore how light propagates from thin elements into a volume for viewing. In particular, devices that are typically connected with geometric optics, like parallax barriers, differ in treatment with those that obey physical optics, like holograms. However, the two concepts are often used to achieve the same effect of capturing or displaying a combination of spatial and angular information. This paper attempts to connect the two approaches under a general framework based in ray space, from which insights into applications and limitations of both parallax-based and holography-based systems can be observed. We show that each display form can generate a light distribution that can always be expressed as a rank-1 matrix. Knowledge of this limitation is then discussed in the context of extending the capabilities of current display forms by considering the use of partially coherent light.

==> rankcomparison__Roarke_Horstmeyer_s_conflicted_copy_2010-01-15_.tex <==
% !TEX root = ./template.tex

\subsection{Rank Comparison of Hologram and Parallax Barrier Outputs}

Although (equations above) will quickly lead us to a phase-space representation for a hologram, they are only meaningful if nice coherent light is used.  An incoherent parallax barrier operates under geometric optics assumptions, given by a light field. The connection between the Wigner distribution and a light field becomes clear when the wavelength of light becomes very small ~\shortcite{Foley1985236}. In this realm, the effects of diffraction become negligible and the original Wigner distribution turns into Walther's radiance function B ~\shortcite{Kim:87} in the small angle approximation: 
\begin{equation}
B = (\frac{1}{\lambda^{2}})W(x,\frac{\theta}{\lambda}),
\end{equation}
which is based on rays with an assigned coordinate x and a unit direction u in 1D. This is equivalent to defining a windowed Wigner distribution based on spatial frequencies, typically tied to an observable quasi light field (Accardi), and setting it to a delta function: 
\begin{equation}
l_{wigner}(x,u)=W\left(x,\frac{\theta}{\lambda}\right)*W_{aperture}\left(-x,\frac{u}{\lambda}\right) \rightarrow W\left(x,\frac{u}{\lambda}\right)*\delta = l
\end{equation} 
This equality holds as long as the limits of the Fourier uncertainty relation are obeyed. As with the two forms of 3D display, this equation implies that the light field and Wigner are applicable at different scales. A light field, like a parallax barrier, works well when variables are much larger than the light wavelength. Neglecting the impact of a finite wavelegth, a Wigner distribution turns into a light field.
  
Consequences of working at the geometric limit in phase space are summarized in the lower portion of Table 1. As noted  above, one important consequence is a limitation to positive values. A simple way to think about this limitation is in Fig. x. Another consequence appears at the interface of light upon a thin element. With no diffraction, a single ray entering a thin element will produce a single ray as an output (Bastiaans). With amplitude-only elements typical of parallax displays, the angle of a ray cannot be changed, which reduces the convolution in (equation above) to a multiplication:
\begin{equation}
l_{3}(x,u)=l_{1} * \delta_{u}(l_{2}) =l_{1}(x,u) l_{2}(x).
\end{equation}

Considering the screen of a parallax barrier $s$ and the barrier mask $m$, the screen will create a broadband light field that propagates a distance $d$ to $m$. Using the shear relation in (equation), We can write $l_{3}(x,\theta)$ in terms of a sheared $s$,
\begin{equation}
l_{3}(x,\theta)= m(x) s(x-d\theta)
\end{equation}

Thus, we see that the 2D light field from two amplitude planes is an outer product of 1D real column vectors:
 \begin{equation}
<m(x_{1})|s(x_{2})>=[LF_{two planes}]
\end{equation}

This matrix has rank 1, which is quite a resrtictive property. This decomposition is most clear when we present the light field in a rotated coordinate system, where the mask functions $m(x)$ and $s(x)$ are the axes (Figure). Discrete lines of angular content $u$ at 45 degrees represent rays from different angles $\theta$ from $s$ through the relationship, 
\begin{equation}
u=d\times\theta
\end{equation}
This implies that a parallax barrier undersamples any higher-rank light field it is designed to approximate. To avoid aliasing, it must sample the light field at large spatial intervals.  
 
Ray angles can change when diffraction effects are permitted, especially under illumination conditions that are partially coherent. So, an equivalent decomposition of two planes under physical optics assumptions will lead to a matrix with full rank in Wigner distribution space: 
\begin{equation}
[W1] * |_{u} [W2] = [W3]
\end{equation}
However, the Wigner distribution for a hologram under coherent plane-wave illumination can always be inverted to determine the original transparency it was generated by: 
\begin{equation}
t(x')t^{*}(0)=\int W(\frac{x'}{2},u) e^{2 \pi i x' u}du
\end{equation}
Thus, up to a constant phase factor, a holographic image also can be decomposed into an outer product relationship similar to (equation above) in a new coordinate space, given that it can be represented by a Wigner distribution. The rank-1 matrix is in a space that is also rotated by 45 degrees, called the mutual-intensity space. The rank-1 property holds for any coherent wavefront distribution after any propagation or modulation by multiple amplitude screens. 





\begin{figure}[htb]
  \centering
  \includegraphics[width=.95\linewidth]{Figures2/Fig8.pdf}

  \caption{\label{fig:firstExample}
           The operation of a thin mask under geometric optics considerations and under physical optics considerations. A ray passing through a slit is convolved with a delta function (vertical slice of a horizontal bar in phase space). The same slice through the Wigner distribution leads to a function of finite width Wm. Convolution with this function leads to a diffraction blur that is independent of incoming ray angle. }
\end{figure}




\begin{figure}[htb]
  \centering
  \includegraphics[width=.95\linewidth]{Figures2/Fig9.pdf}

  \caption{\label{fig:firstExample}
           A simple explanation to why negative values are not available in a geometric optics phase space. (a) The Wigner distribution has negative values under interference conditions, i.e. between two slits. (b) Negative terms are always localized and surrounded by positive values. Putting a soda straw between two slits, no "negative light" will be observable because the positive and negative values will always cancel. (c) The same cancelation can be imagined as a result of scale. Combining 100 hologram pixels to create a parallax barrier pixel will also blur out any negative values that could be used in phase space. }
\end{figure}



\begin{figure}[htb]
  \centering
  \includegraphics[width=.95\linewidth]{Figures2/Fig10.pdf}

  \caption{\label{fig:firstExample}
           A connection between the angular content of the Wigner distribution of a mask and that of a parallax display. Integrating the distribution along x yields the intensity of the frequency spectrum. Integration along u gives the aperture function. The frequency spectrum is similar in function to the angular content of a parallax barrier display behind one slit. }
\end{figure}

